Measurement of the cosmic muon annual and diurnal flux variation with the COSINE-100 detector

We report measurements of annual and diurnal modulations of the cosmic-ray muon rate in the Yangyang underground laboratory (Y2L) using 952 days of COSINE-100 data acquired between September 2016 and July 2019. A correlation of the muon rate with the atmospheric temperature is observed and its amplitude on the muon rate is determined. The effective atmospheric temperature and muon rate variations are positively correlated with a measured effective temperature coefficient of $\alpha_{T}$ = 0.80 $\pm$ 0.11. This result is consistent with a model of meson production in the atmosphere. We also searched for a diurnal modulation in the underground muon rate by comparing one-hour intervals. No significant diurnal modulation of the muon rate was observed.

==> Makefile <==
main:
	pdflatex muonmodulation

sup:
	pdflatex supplementary
	bibtex supplementary
	pdflatex supplementary
	pdflatex supplementary

full:
	pdflatex muonmodulation
	bibtex muonmodulation
	pdflatex muonmodulation
	pdflatex muonmodulation

submit:
	sed -f submit.sed < muonmodulation.tex > muonmodulation_submit.tex
	pdflatex muonmodulation_submit
	pdflatex muonmodulation_submit

clean:
	rm *-converted-to.pdf muonmodulation*.pdf *.aux *.bbl *.blg *.dvi *.log *.toc *.lof *.lot *.out *~ \#*\# *Notes.bib 

